Are Semi-Dense Detector-Free Methods Good at Matching Local Features?

Semi-dense detector-free approaches (SDF), such as LoFTR, are currently among the most popular image matching methods. While SDF methods are trained to establish correspondences between two images, their performances are almost exclusively evaluated using relative pose estimation metrics. Thus, the link between their ability to establish correspondences and the quality of the resulting estimated pose has thus far received little attention. This paper is a first attempt to study this link. We start with proposing a novel structured attention-based image matching architecture (SAM). It allows us to show a counter-intuitive result on two datasets (MegaDepth and HPatches): on the one hand SAM either outperforms or is on par with SDF methods in terms of pose/homography estimation metrics, but on the other hand SDF approaches are significantly better than SAM in terms of matching accuracy. We then propose to limit the computation of the matching accuracy to textured regions, and show that in this case SAM often surpasses SDF methods. Our findings highlight a strong correlation between the ability to establish accurate correspondences in textured regions and the accuracy of the resulting estimated pose/homography. Our code will be made available.

==> 6_conclusion.tex <==
\section{Conclusion\label{sec:conclusion}}


We proposed a novel Structured Attention-based image Matching architecture (\poda). The flexibility of this novel architecture allowed us to fairly compare it against \adf{} methods, \emph{i.e.}, in all the experiments we used the same query locations (source grid with stride
8). The experiments highlighted a counter-intuitive result on two datasets (MegaDepth and HPatches): on the one hand \poda{} either outperforms or is on par with \adf{} methods in terms of pose/homography estimation metrics, but on the other hand \adf{} approaches are significantly better than \poda{} in terms of Matching Accuracy (\ap{}). Here the \ap{} is computed on all the semi-dense locations of the source image with available ground truth correspondent, which includes both textured and uniform regions. 
We proposed to limit the computation of the matching accuracy to textured regions, and showed that in this case \poda{} often surpasses \adf{} methods. These findings highlighted a strong correlation between the ability to establish precise correspondences in textured regions and the accuracy of the resulting estimated pose/homography. We also evaluated the aforementioned methods on ETH3D which confirmed, on a third dataset, that \poda{} has a strong ability to establish correspondences in textures regions. We finally performed an ablation study of \poda{} to demonstrate that each part of the architecture is important to obtain such a strong matching capacity. 


\section*{Acknowledgments}
This project has received funding from the French minist\`ere de l'Enseignement sup\'erieur, de la Recherche et de l'Innovation.
This work was granted access to the HPC resources of IDRIS under the allocation 2022-AD011012858 made by GENCI.





==> sec/3_on_demand.tex <==
\begin{comment}
    
\section{On-demand matching paradigm}\label{sec:odm}

The ability of \adf{} methods to match local features is thoroughly evaluated against \func{} methods, in Sec.~\ref{sec:exp}, \red{and shows that \adf{} architectures are generally %systematically 
outperformed (see \eg Tab.~\ref{table:megadepth_tab}). 
However, the results also indicate that the \func{} approaches, especially COTR, have an unreasonable computational time.}
This observation raises the following question: \red{Is it possible to design an architecture that reaches similar performances, with a reasonable run time?} 
To address this question, we first need to formalize the \odfm{} paradigm.

\mv{
\begin{itemize}
    %\item Avoid "systematically", "outperformed", even if true. More neutral formulation.
    \item The question raised is not related to this section. It may make you think that we design this paradigm because it works better for our architecture.
    \item Reformulate to make it clear that this paradigm it a good evaluation of the feature matching performances of any architecture.
\end{itemize}
}

\subsection{Definition}

Given a set of \mv{L} \red{2D} query locations $\curl{\vp_{\text{s},i}}_{i=1...L}$ in a source image $\mI_\text{s}$, \odfm{} consists in finding their \mv{L} \red{2D} correspondent locations $\curl{\hat{\vp}_{\text{t},i}}_{i=1...L}$  in a target image $\mI_\text{t}$.
Thus a method $\mathcal{M}$ that implements \odfm{} can be written as follows:
\begin{align}
\curl{\hat{\vp}_{\text{t},i}}_{i=1...L}=\mathcal{M}\parr{\mI_{\text{s}},\mI_{\text{t}},\curl{\vp_{\text{s},i}}_{i=1...L}}.\label{eq:odfm}
\end{align}
Let us highlight that \adf{} and \func{} approaches can be viewed as two extreme implementations of \odfm{}. 
A \func{} method implements \odfm{} by predicting the $L$ correspondents $\curl{\hat{\vp}_{\text{t},i}}_{i=1...L}$ of $\curl{\vp_{\text{s},i}}_{i=1...L}$ \emph{independently}. 
This is an extreme implementation as, on the one hand, it makes the approach elegant, but on the other hand, it makes the computational time unreasonable. 
An \adf{} approach can be used to implement \odfm{} since its coarse attention-based matching stage produces dense features for the source and target images. 
Let us recall that at training time, these features are used to compute a coarse 4D correlation volume using a simple dot product between the source and target features to produce coarse dense correspondences. 
Thus, in the \odfm{} context, for each query $\vp_{\text{s},i}$, a feature vector can be interpolated at location $\vp_{\text{s},i}$ in the source features, and a simple dot product between this feature vector and the target features allows one to find a coarse correspondent $\hat{\vp}_{\text{t},i}$. 
This correspondence can then be refined by the fine matching stage. 
This implementation of \odfm{} seems also extreme as it consists in solving the problem for every  source image pixels (at a coarse resolution), and then just querying the results for the $L$ query locations using a simple dot product. 
\red{This analysis will help us to consider a network architecture \red{significantly} different from both \adf{} and \func{} architectures.} \mv{May suggest POD $\implies$ ODM. Reformulate more ODM centered.}

\subsection{Test set}\label{sec:testset}

In order to evaluate the performance of a given method that implements \odfm{}, pairs of source/target images $\curl{\mI_{\text{s}_k},\mI_{\text{t}_k}}_{k=1...K}$ with sets of ground truth correspondences $\curl{\vp_{\text{s}_k,i},\vp_{\text{t}_k,i}}_{i=1...L_k}$ are needed. 
However,  \red{some} \mv{special} care must be taken with the sets of ground truth correspondences. 
For a given query location $\vp_{\text{s}_k,i}$, its correspondent $\vp_{\text{t}_k,i}$ might be 1) outside the target image, 2) occluded or 3) covisible. 
On the one hand, we are mainly interested in evaluating the ability of a given method to find the correspondent $\vp_{\text{t}_k,i}$ of $\vp_{\text{s}_k,i}$, when $\vp_{\text{t}_k,i}$ is \emph{covisible}. 
This would speak in favor of building a test set where each $\vp_{\text{t}_k,i}$ is covisible in the target image. 
On the other hand, building a test set where each $\vp_{\text{t}_k,i}$ is covisible in the target image implies that each $\vp_{\text{s}_k,i}$ conveys a \emph{covisibility} information (see eq.~\ref{eq:odfm}) as input to the method, \ie it indicates the region of the source image that overlaps with the target image. 
Thus, an architecture that is tailored for \odfm{} \red{(as the architecture we propose in Sec.~\ref{sec:method}) could leverage that additional information, while \adf{} and \func{} architectures can not. 
This would lead to unfair comparisons.} \mv{Reformulate : To avoid this bias and for fair comparaison ...}
To prevent the query locations $\curl{\vp_{\text{s},i}}_{i=1...L}$ to convey this information, we opt for a test set where each $\vp_{\text{t}_k,i}$ may or may not be covisible, and add a binary covisibility variable $v_{\text{t}_k,i}$, where $\croch{v_{\text{t}_k,i}=1}$ indicates that $\vp_{\text{t}_k,i}$ is covisible in the target image ($\croch{\cdot}$ is the Iverson bracket). 
More precisely, in practice, for each image pair of each test set, we set $L_k$ to 64 and randomly sample (uniformly) the number of covisible correspondences between 1 and 32. Consequently, a test set can be defined as follows: 
\begin{align}
\mathcal{D_{\text{test}}}=\curl{\mI_{\text{s}_k},\mI_{\text{t}_k},\curl{\vp_{\text{s}_k,i},\vp_{\text{t}_k,i},v_{\text{t}_k,i}}_{i=1...L_k}}_{k=1...K}.\label{eq:testset}
\end{align}

\end{comment}
